Seeing Like an AI: How LLMs Apply (and Misapply) Wikipedia Neutrality Norms

Large language models (LLMs) are trained on broad corpora and then used in communities with specialized norms. Is providing LLMs with community rules enough for models to follow these norms? We evaluate LLMs' capacity to detect (Task 1) and correct (Task 2) biased Wikipedia edits according to Wikipedia's Neutral Point of View (NPOV) policy. LLMs struggled with bias detection, achieving only 64% accuracy on a balanced dataset. Models exhibited contrasting biases (some under- and others over-predicted bias), suggesting distinct priors about neutrality. LLMs performed better at generation, removing 79% of words removed by Wikipedia editors. However, LLMs made additional changes beyond Wikipedia editors' simpler neutralizations, resulting in high-recall but low-precision editing. Interestingly, crowdworkers rated AI rewrites as more neutral (70%) and fluent (61%) than Wikipedia-editor rewrites. Qualitative analysis found LLMs sometimes applied NPOV more comprehensively than Wikipedia editors but often made extraneous non-NPOV-related changes (such as grammar). LLMs may apply rules in ways that resonate with the public but diverge from community experts. While potentially effective for generation, LLMs may reduce editor agency and increase moderation workload (e.g., verifying additions). Even when rules are easy to articulate, having LLMs apply them like community members may still be difficult.

==> images/con_logit_fluent.tex <==

% Table created by stargazer v.5.2.3 by Marek Hlavac, Social Policy Institute. E-mail: marek.hlavac at gmail.com
% Date and time: Sat, Jun 22, 2024 - 21:46:44
\begin{table}[!htbp] \centering 
  \caption{Conditional logistic regression models with coefficients and SEs in parentheses. Variables aside from condition are z-scored, and coefficients be interpreted as a change in the log-odds of being selected associated with a +1 SD increase in the predictor.} 
  \label{con_logit_fluent} 
\tiny 
\begin{tabular}{@{\extracolsep{1pt}}lcccccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{6}{c}{Is Chosen as Most Fluent} \\ 
\cline{2-7} 
\\[-1.8ex] & \multicolumn{6}{c}{} \\ 
\\[-1.8ex] & (1) & (2) & (3) & (4) & (5) & (6)\\ 
\hline \\[-1.8ex] 
 AI: ZeroShot & 0.613$^{***}$ & 0.726$^{***}$ & 0.614$^{***}$ & 0.703$^{***}$ & 0.837$^{***}$ & 0.827$^{***}$ \\ 
  & (0.077) & (0.080) & (0.081) & (0.083) & (0.093) & (0.098) \\ 
  & & & & & & \\ 
 AI: CAI & 0.276$^{***}$ & 0.544$^{***}$ & 0.279$^{***}$ & 0.474$^{***}$ & 0.625$^{***}$ & 0.625$^{***}$ \\ 
  & (0.075) & (0.090) & (0.106) & (0.113) & (0.122) & (0.127) \\ 
  & & & & & & \\ 
 Word count &  & $-$0.904$^{***}$ &  & $-$0.935$^{***}$ & $-$0.748$^{***}$ & $-$0.699$^{**}$ \\ 
  &  & (0.162) &  & (0.165) & (0.172) & (0.335) \\ 
  & & & & & & \\ 
 Number of diffs &  &  & $-$0.003 & 0.058 & 0.097$^{*}$ & 0.058 \\ 
  &  &  & (0.054) & (0.056) & (0.057) & (0.062) \\ 
  & & & & & & \\ 
 Removals as Prop. Of diffs &  &  &  &  & 0.183$^{***}$ & 0.190$^{***}$ \\ 
  &  &  &  &  & (0.051) & (0.057) \\ 
  & & & & & & \\ 
 Six-letter words &  &  &  &  &  & 0.322 \\ 
  &  &  &  &  &  & (0.205) \\ 
  & & & & & & \\ 
 Flesch-Kincaid &  &  &  &  &  & $-$0.083 \\ 
  &  &  &  &  &  & (0.126) \\ 
  & & & & & & \\ 
 Grammar Errors &  &  &  &  &  & $-$0.857$^{***}$ \\ 
  &  &  &  &  &  & (0.177) \\ 
  & & & & & & \\ 
 Average word length &  &  &  &  &  & $-$0.084 \\ 
  &  &  &  &  &  & (0.179) \\ 
  & & & & & & \\ 
 Number of hedges &  &  &  &  &  & $-$0.161$^{**}$ \\ 
  &  &  &  &  &  & (0.074) \\ 
  & & & & & & \\ 
 LIWC Cognitive Words &  &  &  &  &  & $-$0.382$^{***}$ \\ 
  &  &  &  &  &  & (0.116) \\ 
  & & & & & & \\ 
 LIWC Conjunctions &  &  &  &  &  & $-$0.010 \\ 
  &  &  &  &  &  & (0.100) \\ 
  & & & & & & \\ 
\hline \\[-1.8ex] 
Observations & 2,940 & 2,940 & 2,940 & 2,940 & 2,940 & 2,940 \\ 
R$^{2}$ & 0.027 & 0.037 & 0.027 & 0.038 & 0.042 & 0.054 \\ 
Max. Possible R$^{2}$ & 0.500 & 0.500 & 0.500 & 0.500 & 0.500 & 0.500 \\ 
Log Likelihood & $-$978.853 & $-$962.857 & $-$978.852 & $-$962.321 & $-$955.961 & $-$937.290 \\ 
Wald Test & 77.010$^{***}$ (df = 2) & 105.140$^{***}$ (df = 3) & 77.010$^{***}$ (df = 3) & 105.810$^{***}$ (df = 4) & 115.240$^{***}$ (df = 5) & 141.500$^{***}$ (df = 12) \\ 
LR Test & 80.146$^{***}$ (df = 2) & 112.139$^{***}$ (df = 3) & 80.149$^{***}$ (df = 3) & 113.211$^{***}$ (df = 4) & 125.930$^{***}$ (df = 5) & 163.274$^{***}$ (df = 12) \\ 
Score (Logrank) Test & 79.104$^{***}$ (df = 2) & 109.774$^{***}$ (df = 3) & 79.106$^{***}$ (df = 3) & 110.701$^{***}$ (df = 4) & 122.310$^{***}$ (df = 5) & 155.654$^{***}$ (df = 12) \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{6}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular} 
\end{table} 


==> tables/acc_topic.tex <==
\begin{table}[h]
\centering
\begin{tabular}{lrrr}
\toprule
{} &  Mean &  Lower Bound &  Upper Bound \\
\midrule
Assistance          &  0.55 &         0.52 &         0.58 \\
Culture             &  0.64 &         0.61 &         0.67 \\
Geography           &  0.53 &         0.50 &         0.56 \\
History And Society &  0.57 &         0.54 &         0.60 \\
STEM                &  0.61 &         0.58 &         0.64 \\
\bottomrule
\end{tabular}
\caption{Accuracy by topic, displaying lower and upper bound of 95\% CIs.}
\label{acc_table_topic}
\end{table}


==> tables/ai_removal_multi.tex <==
\begin{table}
\centering
\begin{tabular}{llllrlll}
\toprule
Prompt Type & Is Constrained & Precision & Recall &   F1 & Similarity & Non Disjoint & BLEU \\
\midrule
        CAI &              N &      0.27 &   0.86 & 0.41 &       0.26 &         0.93 & 0.21 \\
        CAI &              Y &      0.35 &   0.79 & 0.48 &       0.32 &         0.89 & 0.42 \\
   ZeroShot &              N &      0.37 &   0.75 & 0.49 &       0.33 &         0.85 & 0.46 \\
   ZeroShot &              Y &      0.47 &   0.65 & 0.55 &       0.40 &         0.79 & 0.62 \\
\bottomrule
\end{tabular}
\caption{To rule out that our findings were dependent on the analytical choices we made, we re-ran this analysis multiple times under different analytic decisions. For each condition and metric, we calculcate the mean across 32 ways of conducting this analysis. We varied (1) whether undefined precision calculcations were treated as zero or missing, (2) whether undefined recall calculcations were treated as zero or missing, (3) whether or not diff-based metrics stripped punctuation, (4) whether or not diff-based metrics stripped stop-words or not, and whether BLEU scores were calculcated with smoothing. Results are very similar to results reported in the body of the paper.}
\label{ai_removal_multi}
\end{table}


==> tables/classification_ChatGPT_3.5_FewShot_Minimal.tex <==
\begin{table}
\centering
\begin{tabular}{lrrrr}
\toprule
{} &  precision &  recall &  f1-score &  support \\
\midrule
0            &       0.57 &    0.51 &      0.54 &   150.00 \\
1            &       0.55 &    0.61 &      0.58 &   150.00 \\
accuracy     &       0.56 &    0.56 &      0.56 &   300.00 \\
macro avg    &       0.56 &    0.56 &      0.56 &   300.00 \\
weighted avg &       0.56 &    0.56 &      0.56 &   300.00 \\
\bottomrule
\end{tabular}
\caption{Classification report for: Model==ChatGPT 3.5, Examples==FewShot, Prompt==Minimal}
\label{classification_ChatGPT 3.5_FewShot_Minimal}
\end{table}


==> tables/classification_ChatGPT_3.5_FewShot_NPOV.tex <==
\begin{table}
\centering
\begin{tabular}{lrrrr}
\toprule
{} &  precision &  recall &  f1-score &  support \\
\midrule
0            &       0.57 &    0.43 &      0.49 &   148.00 \\
1            &       0.54 &    0.68 &      0.60 &   149.00 \\
accuracy     &       0.55 &    0.55 &      0.55 &   297.00 \\
macro avg    &       0.56 &    0.55 &      0.54 &   297.00 \\
weighted avg &       0.56 &    0.55 &      0.54 &   297.00 \\
\bottomrule
\end{tabular}
\caption{Classification report for: Model==ChatGPT 3.5, Examples==FewShot, Prompt==NPOV}
\label{classification_ChatGPT 3.5_FewShot_NPOV}
\end{table}


==> tables/classification_ChatGPT_3.5_FewShot_NPOVScoped.tex <==
\begin{table}
\centering
\begin{tabular}{lrrrr}
\toprule
{} &  precision &  recall &  f1-score &  support \\
\midrule
0            &       0.58 &    0.48 &      0.53 &   149.00 \\
1            &       0.56 &    0.65 &      0.60 &   150.00 \\
accuracy     &       0.57 &    0.57 &      0.57 &   299.00 \\
macro avg    &       0.57 &    0.57 &      0.57 &   299.00 \\
weighted avg &       0.57 &    0.57 &      0.57 &   299.00 \\
\bottomrule
\end{tabular}
\caption{Classification report for: Model==ChatGPT 3.5, Examples==FewShot, Prompt==NPOVScoped}
\label{classification_ChatGPT 3.5_FewShot_NPOVScoped}
\end{table}


==> tables/classification_ChatGPT_3.5_ZeroShot_Minimal.tex <==
\begin{table}
\centering
\begin{tabular}{lrrrr}
\toprule
{} &  precision &  recall &  f1-score &  support \\
\midrule
0            &       0.66 &    0.30 &      0.41 &   149.00 \\
1            &       0.55 &    0.85 &      0.66 &   150.00 \\
accuracy     &       0.57 &    0.57 &      0.57 &   299.00 \\
macro avg    &       0.60 &    0.57 &      0.54 &   299.00 \\
weighted avg &       0.60 &    0.57 &      0.54 &   299.00 \\
\bottomrule
\end{tabular}
\caption{Classification report for: Model==ChatGPT 3.5, Examples==ZeroShot, Prompt==Minimal}
\label{classification_ChatGPT 3.5_ZeroShot_Minimal}
\end{table}


==> tables/classification_ChatGPT_3.5_ZeroShot_NPOV.tex <==
\begin{table}
\centering
\begin{tabular}{lrrrr}
\toprule
{} &  precision &  recall &  f1-score &  support \\
\midrule
0            &       0.59 &    0.17 &      0.27 &   149.00 \\
1            &       0.52 &    0.88 &      0.65 &   150.00 \\
accuracy     &       0.53 &    0.53 &      0.53 &   299.00 \\
macro avg    &       0.55 &    0.53 &      0.46 &   299.00 \\
weighted avg &       0.55 &    0.53 &      0.46 &   299.00 \\
\bottomrule
\end{tabular}
\caption{Classification report for: Model==ChatGPT 3.5, Examples==ZeroShot, Prompt==NPOV}
\label{classification_ChatGPT 3.5_ZeroShot_NPOV}
\end{table}


==> tables/classification_ChatGPT_3.5_ZeroShot_NPOVScoped.tex <==
\begin{table}
\centering
\begin{tabular}{lrrrr}
\toprule
{} &  precision &  recall &  f1-score &  support \\
\midrule
0            &       0.61 &    0.18 &      0.28 &   150.00 \\
1            &       0.52 &    0.89 &      0.66 &   150.00 \\
accuracy     &       0.53 &    0.53 &      0.53 &   300.00 \\
macro avg    &       0.57 &    0.53 &      0.47 &   300.00 \\
weighted avg &       0.57 &    0.53 &      0.47 &   300.00 \\
\bottomrule
\end{tabular}
\caption{Classification report for: Model==ChatGPT 3.5, Examples==ZeroShot, Prompt==NPOVScoped}
\label{classification_ChatGPT 3.5_ZeroShot_NPOVScoped}
\end{table}


==> tables/classification_GPT-4_FewShot_Minimal.tex <==
\begin{table}
\centering
\begin{tabular}{lrrrr}
\toprule
{} &  precision &  recall &  f1-score &  support \\
\midrule
0            &       0.61 &    0.63 &      0.62 &   150.00 \\
1            &       0.62 &    0.59 &      0.61 &   150.00 \\
accuracy     &       0.61 &    0.61 &      0.61 &   300.00 \\
macro avg    &       0.61 &    0.61 &      0.61 &   300.00 \\
weighted avg &       0.61 &    0.61 &      0.61 &   300.00 \\
\bottomrule
\end{tabular}
\caption{Classification report for: Model==GPT-4, Examples==FewShot, Prompt==Minimal}
\label{classification_GPT-4_FewShot_Minimal}
\end{table}


==> tables/classification_GPT-4_FewShot_NPOV.tex <==
\begin{table}
\centering
\begin{tabular}{lrrrr}
\toprule
{} &  precision &  recall &  f1-score &  support \\
\midrule
0            &       0.60 &    0.56 &      0.58 &   150.00 \\
1            &       0.58 &    0.62 &      0.60 &   150.00 \\
accuracy     &       0.59 &    0.59 &      0.59 &   300.00 \\
macro avg    &       0.59 &    0.59 &      0.59 &   300.00 \\
weighted avg &       0.59 &    0.59 &      0.59 &   300.00 \\
\bottomrule
\end{tabular}
\caption{Classification report for: Model==GPT-4, Examples==FewShot, Prompt==NPOV}
\label{classification_GPT-4_FewShot_NPOV}
\end{table}


==> tables/classification_GPT-4_FewShot_NPOVScoped.tex <==
\begin{table}
\centering
\begin{tabular}{lrrrr}
\toprule
{} &  precision &  recall &  f1-score &  support \\
\midrule
0            &       0.60 &    0.57 &      0.58 &   150.00 \\
1            &       0.59 &    0.63 &      0.61 &   150.00 \\
accuracy     &       0.60 &    0.60 &      0.60 &   300.00 \\
macro avg    &       0.60 &    0.60 &      0.60 &   300.00 \\
weighted avg &       0.60 &    0.60 &      0.60 &   300.00 \\
\bottomrule
\end{tabular}
\caption{Classification report for: Model==GPT-4, Examples==FewShot, Prompt==NPOVScoped}
\label{classification_GPT-4_FewShot_NPOVScoped}
\end{table}


==> tables/classification_GPT-4_ZeroShot_Minimal.tex <==
\begin{table}
\centering
\begin{tabular}{lrrrr}
\toprule
{} &  precision &  recall &  f1-score &  support \\
\midrule
0            &       0.57 &    0.71 &      0.63 &   149.00 \\
1            &       0.62 &    0.47 &      0.54 &   150.00 \\
accuracy     &       0.59 &    0.59 &      0.59 &   299.00 \\
macro avg    &       0.60 &    0.59 &      0.59 &   299.00 \\
weighted avg &       0.60 &    0.59 &      0.59 &   299.00 \\
\bottomrule
\end{tabular}
\caption{Classification report for: Model==GPT-4, Examples==ZeroShot, Prompt==Minimal}
\label{classification_GPT-4_ZeroShot_Minimal}
\end{table}


==> tables/classification_GPT-4_ZeroShot_NPOV.tex <==
\begin{table}
\centering
\begin{tabular}{lrrrr}
\toprule
{} &  precision &  recall &  f1-score &  support \\
\midrule
0            &       0.66 &    0.54 &      0.59 &   148.00 \\
1            &       0.61 &    0.71 &      0.66 &   147.00 \\
accuracy     &       0.63 &    0.63 &      0.63 &   295.00 \\
macro avg    &       0.63 &    0.63 &      0.62 &   295.00 \\
weighted avg &       0.63 &    0.63 &      0.62 &   295.00 \\
\bottomrule
\end{tabular}
\caption{Classification report for: Model==GPT-4, Examples==ZeroShot, Prompt==NPOV}
\label{classification_GPT-4_ZeroShot_NPOV}
\end{table}


==> tables/classification_GPT-4_ZeroShot_NPOVScoped.tex <==
\begin{table}
\centering
\begin{tabular}{lrrrr}
\toprule
{} &  precision &  recall &  f1-score &  support \\
\midrule
0            &       0.62 &    0.58 &      0.60 &   147.00 \\
1            &       0.61 &    0.65 &      0.63 &   148.00 \\
accuracy     &       0.61 &    0.61 &      0.61 &   295.00 \\
macro avg    &       0.61 &    0.61 &      0.61 &   295.00 \\
weighted avg &       0.61 &    0.61 &      0.61 &   295.00 \\
\bottomrule
\end{tabular}
\caption{Classification report for: Model==GPT-4, Examples==ZeroShot, Prompt==NPOVScoped}
\label{classification_GPT-4_ZeroShot_NPOVScoped}
\end{table}


==> tables/classification_MistralMedium_FewShot_Minimal.tex <==
\begin{table}
\centering
\begin{tabular}{lrrrr}
\toprule
{} &  precision &  recall &  f1-score &  support \\
\midrule
0            &       0.58 &    0.77 &      0.66 &   149.00 \\
1            &       0.66 &    0.46 &      0.54 &   149.00 \\
accuracy     &       0.61 &    0.61 &      0.61 &   298.00 \\
macro avg    &       0.62 &    0.61 &      0.60 &   298.00 \\
weighted avg &       0.62 &    0.61 &      0.60 &   298.00 \\
\bottomrule
\end{tabular}
\caption{Classification report for: Model==MistralMedium, Examples==FewShot, Prompt==Minimal}
\label{classification_MistralMedium_FewShot_Minimal}
\end{table}


==> tables/classification_MistralMedium_FewShot_NPOV.tex <==
\begin{table}
\centering
\begin{tabular}{lrrrr}
\toprule
{} &  precision &  recall &  f1-score &  support \\
\midrule
0            &       0.57 &    0.54 &      0.56 &   149.00 \\
1            &       0.57 &    0.60 &      0.58 &   149.00 \\
accuracy     &       0.57 &    0.57 &      0.57 &   298.00 \\
macro avg    &       0.57 &    0.57 &      0.57 &   298.00 \\
weighted avg &       0.57 &    0.57 &      0.57 &   298.00 \\
\bottomrule
\end{tabular}
\caption{Classification report for: Model==MistralMedium, Examples==FewShot, Prompt==NPOV}
\label{classification_MistralMedium_FewShot_NPOV}
\end{table}


==> tables/classification_MistralMedium_FewShot_NPOVScoped.tex <==
\begin{table}
\centering
\begin{tabular}{lrrrr}
\toprule
{} &  precision &  recall &  f1-score &  support \\
\midrule
0            &       0.58 &    0.56 &      0.57 &   146.00 \\
1            &       0.57 &    0.59 &      0.58 &   146.00 \\
accuracy     &       0.58 &    0.58 &      0.58 &   292.00 \\
macro avg    &       0.58 &    0.58 &      0.58 &   292.00 \\
weighted avg &       0.58 &    0.58 &      0.58 &   292.00 \\
\bottomrule
\end{tabular}
\caption{Classification report for: Model==MistralMedium, Examples==FewShot, Prompt==NPOVScoped}
\label{classification_MistralMedium_FewShot_NPOVScoped}
\end{table}


==> tables/classification_MistralMedium_ZeroShot_Minimal.tex <==
\begin{table}
\centering
\begin{tabular}{lrrrr}
\toprule
{} &  precision &  recall &  f1-score &  support \\
\midrule
0            &       0.55 &    0.83 &      0.66 &   149.00 \\
1            &       0.64 &    0.32 &      0.42 &   149.00 \\
accuracy     &       0.57 &    0.57 &      0.57 &   298.00 \\
macro avg    &       0.60 &    0.57 &      0.54 &   298.00 \\
weighted avg &       0.60 &    0.57 &      0.54 &   298.00 \\
\bottomrule
\end{tabular}
\caption{Classification report for: Model==MistralMedium, Examples==ZeroShot, Prompt==Minimal}
\label{classification_MistralMedium_ZeroShot_Minimal}
\end{table}


==> tables/classification_MistralMedium_ZeroShot_NPOV.tex <==
\begin{table}
\centering
\begin{tabular}{lrrrr}
\toprule
{} &  precision &  recall &  f1-score &  support \\
\midrule
0            &       0.59 &    0.62 &      0.60 &   146.00 \\
1            &       0.61 &    0.57 &      0.59 &   150.00 \\
accuracy     &       0.60 &    0.60 &      0.60 &   296.00 \\
macro avg    &       0.60 &    0.60 &      0.60 &   296.00 \\
weighted avg &       0.60 &    0.60 &      0.60 &   296.00 \\
\bottomrule
\end{tabular}
\caption{Classification report for: Model==MistralMedium, Examples==ZeroShot, Prompt==NPOV}
\label{classification_MistralMedium_ZeroShot_NPOV}
\end{table}


==> tables/classification_MistralMedium_ZeroShot_NPOVScoped.tex <==
\begin{table}
\centering
\begin{tabular}{lrrrr}
\toprule
{} &  precision &  recall &  f1-score &  support \\
\midrule
0            &       0.58 &    0.64 &      0.61 &   145.00 \\
1            &       0.61 &    0.55 &      0.58 &   148.00 \\
accuracy     &       0.59 &    0.59 &      0.59 &   293.00 \\
macro avg    &       0.60 &    0.59 &      0.59 &   293.00 \\
weighted avg &       0.60 &    0.59 &      0.59 &   293.00 \\
\bottomrule
\end{tabular}
\caption{Classification report for: Model==MistralMedium, Examples==ZeroShot, Prompt==NPOVScoped}
\label{classification_MistralMedium_ZeroShot_NPOVScoped}
\end{table}


==> tables/con_logit_fluent.tex <==

% Table created by stargazer v.5.2.3 by Marek Hlavac, Social Policy Institute. E-mail: marek.hlavac at gmail.com
% Date and time: Thu, Dec 19, 2024 - 14:33:59
\begin{table}[!htbp] \centering 
\tiny 
\begin{tabular}{@{\extracolsep{1pt}}lcc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{2}{c}{Is Chosen as Most Fluent} \\ 
\cline{2-3} 
\\[-1.8ex] & \multicolumn{2}{c}{} \\ 
\\[-1.8ex] & (1) & (2)\\ 
\hline \\[-1.8ex] 
 AI: ZeroShot & 0.613$^{***}$ & 0.742$^{***}$ \\ 
  & (0.077) & (0.085) \\ 
  & & \\ 
 AI: CAI & 0.276$^{***}$ & 0.489$^{***}$ \\ 
  & (0.075) & (0.114) \\ 
  & & \\ 
 Word count &  & $-$0.712$^{***}$ \\ 
  &  & (0.172) \\ 
  & & \\ 
 Number of diffs &  & 0.0003 \\ 
  &  & (0.058) \\ 
  & & \\ 
 Grammar Errors &  & $-$0.735$^{***}$ \\ 
  &  & (0.162) \\ 
  & & \\ 
\hline \\[-1.8ex] 
Observations & 2,940 & 2,940 \\ 
R$^{2}$ & 0.027 & 0.045 \\ 
Max. Possible R$^{2}$ & 0.500 & 0.500 \\ 
Log Likelihood & $-$978.853 & $-$951.767 \\ 
Wald Test & 77.010$^{***}$ (df = 2) & 122.210$^{***}$ (df = 5) \\ 
LR Test & 80.146$^{***}$ (df = 2) & 134.319$^{***}$ (df = 5) \\ 
Score (Logrank) Test & 79.104$^{***}$ (df = 2) & 130.089$^{***}$ (df = 5) \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{2}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular} 
\caption{Conditional logistic regression models of fluency with coefficients and SEs in parentheses. Variables aside from condition are z-scored, and coefficients be interpreted as a change in the log-odds of being selected associated with a +1 SD increase in the predictor. Grammar errors were computed using LanguageTool.} 
  \label{con_logit_fluent} 
\end{table} 


==> tables/con_logit_neut.tex <==

% Table created by stargazer v.5.2.3 by Marek Hlavac, Social Policy Institute. E-mail: marek.hlavac at gmail.com
% Date and time: Thu, Dec 19, 2024 - 14:33:58
\begin{table}[!htbp] \centering 
\tiny 
\begin{tabular}{@{\extracolsep{1pt}}lcc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{2}{c}{Is Chosen as Most Neutral} \\ 
\cline{2-3} 
\\[-1.8ex] & \multicolumn{2}{c}{} \\ 
\\[-1.8ex] & (1) & (2)\\ 
\hline \\[-1.8ex] 
 AI: ZeroShot & 0.854$^{***}$ & 0.859$^{***}$ \\ 
  & (0.080) & (0.087) \\ 
  & & \\ 
 AI: CAI & 0.802$^{***}$ & 0.754$^{***}$ \\ 
  & (0.080) & (0.119) \\ 
  & & \\ 
 Word count &  & $-$0.444$^{**}$ \\ 
  &  & (0.179) \\ 
  & & \\ 
 Number of diffs &  & 0.133$^{**}$ \\ 
  &  & (0.062) \\ 
  & & \\ 
 Grammar Errors &  & $-$0.235 \\ 
  &  & (0.165) \\ 
  & & \\ 
\hline \\[-1.8ex] 
Observations & 2,940 & 2,940 \\ 
R$^{2}$ & 0.076 & 0.081 \\ 
Max. Possible R$^{2}$ & 0.500 & 0.500 \\ 
Log Likelihood & $-$902.892 & $-$895.280 \\ 
Wald Test & 213.350$^{***}$ (df = 2) & 221.220$^{***}$ (df = 5) \\ 
LR Test & 232.068$^{***}$ (df = 2) & 247.293$^{***}$ (df = 5) \\ 
Score (Logrank) Test & 225.874$^{***}$ (df = 2) & 238.653$^{***}$ (df = 5) \\ 
\hline 
\hline \\[-1.8ex] 
\textit{Note:}  & \multicolumn{2}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\ 
\end{tabular} 
\caption{Conditional logistic regression models of neutrality with coefficients and SEs in parentheses. Variables aside from condition are z-scored, and coefficients be interpreted as a change in the log-odds of being selected associated with a +1 SD increase in the predictor. Grammar errors were computed using LanguageTool.} 
  \label{con_logit_neut} 
\end{table} 


==> tables/cscw_challenges.tex <==
\begin{table}[]
\begin{tabular}{@{}lll@{}}
\toprule
Level              & Human-AI Challenge(s) & Example Question                                                         \\ \midrule
Micro (Individual) & Agency; Workload      & Does co-writing peer-produced content affect editor agency?              \\
Meso (Community)   & Steerability          & Can commerical LLMs be steered to enforce community-specific violations? \\
Macro (Platform) & Credibility; Bias & How does the perception of AI-generated content on a platform affect trust in content? \\ \bottomrule
\end{tabular}
\caption{Our findings raise several questions about human-AI collaboration in CSCW spaces. }
\label{tab:ai_cscw}
\end{table}


==> tables/desc_stats.tex <==
\begin{table*}[t]
\centering

\begin{minipage}[b]{0.5\linewidth}
\centering
\subcaption{Number of edits for each topic}
\label{tab:topic_counts}
\begin{tabular}{lr}
\toprule
Topic & Count \\
\midrule
Culture & 27423 \\
Geography & 13752 \\
History And Society & 10094 \\
STEM & 4157 \\
Assistance & 60 \\
\textbf{Grand Total} & \textbf{55486} \\
\bottomrule
\end{tabular}
\end{minipage}%
\hfill
\begin{minipage}[b]{0.45\linewidth}
\centering
\subcaption{Descriptive statistics for normalized edit distance of edits eligible for the detection experiment. The normalized edit distance between two strings (0-1) is the edit distance divided by the length of the maximum string.}
\label{tab:norm_dist_stats}
\begin{tabular}{lr}
\toprule
Statistic & Value \\
\midrule
mean & 0.07 \\
std & 0.05 \\
25\% & 0.04 \\
50\% & 0.06 \\
75\% & 0.09 \\
\bottomrule
\end{tabular}
\end{minipage}
\caption{Summary Statistics for Wikipedia Edits}
\label{tab:combined_tables}
\end{table*}

==> tables/distinctive_words.tex <==
\begin{table}[ht]
\small
\begin{tabular}{lr lr lr }
\toprule
implicitly\, & 8.26 & valuation\, & 7.57 & toward\, & 7.28\\
lead\, & 8.13 & subtly\, & 7.57 & outlines\, & 7.28\\
employs\, & 8.13 & narrative\, & 7.44 &  & \\
complexity\, & 8.06 & mislead\, & 7.44 &  & \\
\bottomrule
\end{tabular}
\caption{Top 10 distinctive words in GPT-4 explanations by log odds ratio (shown to the right of each word).}
\label{tab:distinctive-words}
\end{table}

==> tables/gen_stats.tex <==
\begin{table}
\centering
\begin{tabular}{lllll}
\toprule
Prompt Type & Is Constrained & Edit Distance &     N Changes &    Word Count \\
\midrule
        CAI &              N &   0.56 (0.17) & 25.88 (16.75) & 47.27 (28.97) \\
        CAI &              Y &   0.35 (0.17) &  12.94 (9.35) & 30.17 (16.03) \\
   ZeroShot &              N &   0.29 (0.15) &  10.52 (7.67) & 28.65 (15.26) \\
   ZeroShot &              Y &   0.18 (0.12) &   6.18 (5.07) & 28.05 (14.79) \\
\bottomrule
\end{tabular}
\caption{AI edit intensity metrics. These measure how many changes AI models applied to the initial, biased edit.}
\label{ai_gen_stats}
\end{table}


==> tables/manual_annot.tex <==
\begin{table}
\begin{tabular}{lll}
\toprule
Topic & Additions & Removals \\
\midrule
Culture & 3/12 & 3/12 \\
Geography & 6/12 & 0/12 \\
History And Society & 1/12 & 0/12 \\
STEM & 4/12 & 0/12 \\
\bottomrule
\end{tabular}
\caption{Two members of the study team manually annotated 48 for additions and removals.}
\label{manual_annot_hal}
\end{table}


==> tables/regexplanation.tex <==
\begin{table}[!htbp] \centering
\begin{tabular}{@{\extracolsep{5pt}}lc}
\\[-1.8ex]\hline
\hline \\[-1.8ex]
& \multicolumn{1}{c}{\textit{Dependent variable: Accuracy}} \
\cr \cline{2-2}
\\[-1.8ex] & (1) \\
\hline \\[-1.8ex]
 Examples[FewShot] & 1.051$^{}$ \\
& (0.938 , 1.177) \\
 Intercept & 1.098$^{}$ \\
& (0.906 , 1.330) \\
 Model[GPT-4] & 1.351$^{***}$ \\
& (1.155 , 1.578) \\
 Model[MistralMedium] & 1.295$^{***}$ \\
& (1.118 , 1.499) \\
 Prompt[NPOVScoped] & 0.873$^{}$ \\
& (0.736 , 1.037) \\
 Prompt[NPOV] & 0.893$^{}$ \\
& (0.760 , 1.048) \\
 avgwordlength & 0.958$^{}$ \\
& (0.887 , 1.034) \\
 cognitivewords & 0.970$^{}$ \\
& (0.906 , 1.038) \\
 conjunctions & 0.905$^{***}$ \\
& (0.850 , 0.964) \\
 emotionwords & 1.089$^{***}$ \\
& (1.026 , 1.155) \\
 maxoverlap & 0.983$^{}$ \\
& (0.914 , 1.057) \\
 policywords & 1.124$^{***}$ \\
& (1.051 , 1.201) \\
 readinggradelevel & 1.056$^{}$ \\
& (0.981 , 1.137) \\
 roottopic[Culture] & 1.385$^{***}$ \\
& (1.155 , 1.660) \\
 roottopic[Geography] & 0.911$^{}$ \\
& (0.762 , 1.088) \\
 roottopic[HistoryAndSociety] & 1.109$^{}$ \\
& (0.928 , 1.325) \\
 roottopic[STEM] & 1.250$^{**}$ \\
& (1.044 , 1.498) \\
 similaritytoprompt & 1.149$^{***}$ \\
& (1.070 , 1.233) \\
 wordcount & 0.799$^{***}$ \\
& (0.740 , 0.863) \\
\hline \\[-1.8ex]
 Observations & 5085 \\
 Pseudo $R^2$ & 0.022 \\
\hline
\hline \\[-1.8ex]
\textit{Note:} & \multicolumn{1}{r}{$^{*}$p$<$0.1; $^{**}$p$<$0.05; $^{***}$p$<$0.01} \\
\end{tabular}
\caption{Logistic regression predicting accuracy of classifications by explanation features. Non-categorical variables are z-scored so odds ratios are interpreted as the change in odds per standard deviation increase in the predictor. Odds ratios are shown with 95\% CIs in parentheses.}
\label{regexplanation}
\end{table}

==> tables/sum_h_stats.tex <==
\begin{table}
\centering
\begin{tabular}{lllll}
\toprule
Question Type &           Matchup & AI Prop & Human Prop &       Delta \\
\midrule
   Neutrality & Human vs ZeroShot &    0.70 &       0.30 &    0.40**** \\
   Neutrality &      Human vs CAI &    0.69 &       0.31 &    0.38**** \\
      Fluency & Human vs ZeroShot &    0.65 &       0.35 &    0.30**** \\
      Fluency &      Human vs CAI &    0.57 &       0.43 &     0.14*** \\
          Add & Human vs ZeroShot &    0.27 &       0.23 & 0.03 (n.s.) \\
          Add &      Human vs CAI &    0.34 &       0.33 & 0.01 (n.s.) \\
       Remove & Human vs ZeroShot &    0.41 &       0.40 & 0.01 (n.s.) \\
       Remove &      Human vs CAI &    0.42 &       0.40 & 0.02 (n.s.) \\
\bottomrule
\end{tabular}
\caption{Experiment results. For fluency and neutrality, participants chose between an AI and a human edit. P-values are computed using two-tailed binomial tests for whether the probability of picking an AI edit differs from 0.5. For additions and removals, participants evaluated each of the AI and huamn edits seperately. P-values are computed using chi-squared tests on whether human vs AI edits differed in frequencies of adding or removing information. `Delta' is the AI proportion minus the human proportion. Stars: n.s. p>0.05, *p ≤ 0.05, **p≤ 0.01 ***p≤ 0.001, ****p≤ 0.0001}
\label{tab:sum_expr_stats_True.astype(str)}
\end{table}

